Further understanding the interaction between dark energy and dark matter: current status and future directions

The interaction between dark matter and dark energy can be incorporated into field theory models of dark energy that have proved successful in alleviating the coincidence problem. We review recent advances in this field, including new models and constraints from different astronomical data sets. We show that interactions are allowed by observations and can reduce the current tensions among different measurements of cosmological parameters. We extend our discussion to include constraints from non-linear effects and results from cosmological simulations. Finally, we discuss forthcoming multi-messenger data from current and future observational facilities that will help to improve our understanding of the interactions within the dark sector.

==> Chapter_3_Current_constraint.tex <==
%\section{Current constraints and forecasts}
%\subsection{Current constraints on the interacting parameters}
%\subsection{Possible alleviatation in observational tensions observed in the $\Lambda$CDM model}
%\subsection{Sequence of Cosmological eras}
%\subsection{Attractor Solutions of Friedmann models}
%\subsection{Stability of Attractor solutions}
%\subsection{Age of the Universe}


==> acronyms.tex <==
\begin{longtable}{|p{3.5cm}|p{13cm}|}
%\begin{tabular}{|p{3.5cm}|p{13cm}|}
\hline
\multicolumn{2}{|c|}{\bf Coordinates}\\
\hline
$(x^\mu)\equiv (t,x,y,z)$ & space-time coordinates\\
$(x^i)\equiv (x,y,z)$ & spatial coordinates\\
$\tau$ & conformal time\\
$\dot f=df/d\tau$ & conformal time derivative\\
\hline
\multicolumn{2}{|c|}{\bf Metric} \\
\hline
$g_{\mu\nu}$ & four dimentional space-time metric tensor\\
$\gamma_{\mu\nu}$ & spatial part of the metric tensor\\ 
$\kappa$ & spatial curvature \\
	& $\kappa=-1,0,1$ for open, flat and close Friedmann models\\
\hline
\multicolumn{2}{|c|}{\bf Background magnitudes}\\
\hline
$a$ & cosmic scale factor\\
$N=\ln(a)$ & \\
$f^\prime=df/dN$ & derivative with respect \\  
$H$ & Hubble factor: $H=a^{-1}(da/dt)$\\
$\cal{H}$ & conformal Hubble factor: $\cal{H}=a^{-1}\dot{a}=aH$\\
$h$ & Hubble constant in units of $100$kms$^{-1}$Mpc$^{-1}$\\
$\rho$ & total energy density\\
$\Omega$ & density in units of the critical density: $\Omega=\rho/[3H^2/8\pi G]$\\
$P$ & total pressure\\
$w_{eff}$ & effective equation of state parameter: $P=w_{eff}\rho$\\
$\rho_A$ & energy density of the A fluid component\\
$\Omega_A$ & density of the Ath component in units of the critical density\\
$P_A$ & pressure of the A fluid component\\
$w_{A}$ & equation of state parameter of A component: $P_A=w_{A}\rho_A$\\
$c_{s,A}$ & sound speed of the Ath component: $c_{s,A}=\delta P/\delta\rho$\\
$c_{a,A}$ & adiabatic sound speed of the Ath component: $c_{a,A}=\dot{P}/\dot{\rho}$\\
\hline
\multicolumn{2}{|c|}{\bf Metric Perturbations}\\
\hline
$B$ & Perturbation of the shift vector in a general gauge\\
$E$ & Anisotropic distortion of constant time hypersurfaces in a general gauge\\
$\psi$ & Perturbation in the lapse function in a general gauge;\\
       & newtonian potential in the longitudinal gauge\\
$\phi$ & Perturbation in the unit 3-volume in a general gauge;\\
       & scalar potential in the longitudinal gauge\\
$h_{ij}$ & Metric perturbations in the synchronous gauge\\
$h$ & Trace of the metric perturbations in the synchronous gauge\\
$\eta$ & Traceless part of the metric perturbations in the synchronous gauge\\
\hline
\multicolumn{2}{|c|}{\bf Perturbations of Physical Magnitudes}\\
\hline
$\bar{\rho}_A$ & mean (background) density of the Ath fluid component\\
$\delta\rho_A$ & density perturbation \\
$\delta_A$ & density contrast: $\delta_A=\delta\rho_A/\rho_A$\\
$\bar{P}_A$ & mean (background) pressure of the Ath fluid component\\
$P_A$ & pressure perturbation\\
$\pi_A$ & anisotropic perturbation\\
$Q_A^{\mu}$ & Momentum transfered by the DM/DE interaction\\
$Q_A^{\mu}$ & Momentum transfered by the DM/DE interaction\\
\hline
%\end{tabular}
\caption{Symbols most frequently used in the text.}
\end{longtable}


==> bibliography.tex <==
\subsubsection*{Acknowledgements}
F.A.B. acknowledges financial support from Grants
PID2021-122938NB-I00 funded by MCIN/AEI/10.13039/501100011033
and by “ERDF A way of making Europe" and SA083P17 funded by the Junta de Castilla y Le\'on. B. W. acknowledges the support by National Natural Science Foundation of China and discussions with Costa A. and Zhang J. 

%\section{Bibliography}

\begin{thebibliography}{99}

\bibitem{Abbott:2017}
\reference{Abbott~T.~M.~C., et al.}{Phys. Rev. D}{98}{043526}{2018}

%\bibitem{abdalla1}
%\reference{E.~Abdalla, L.~R.~Abramo, L.~Sodre, B.~Wang}{Phys. Lett. B}{673}{107}{2009}

\bibitem{Abdalla:2020}
\reference{Abdalla E and Marins A}{International Journal of Modern Physics D}{\bf 29}{2030014}{2020}

\bibitem{Abdalla2021a}
\reference{Abdalla E, et al.}{Astron. Astrophys.}{664}{A14}{2022}

\bibitem{Abdalla2021b}
\reference{Abdalla F. B., et al.}{Astron. Astrophys.}{664}{A16}{2022}

\bibitem{Abdalla:2022a}
\reference{Abdalla E, Abell\'an G. F., Aboubrahim A et al}{\it Journal of High Energy Astrophysics}{\bf 34}{49}{2022}

\bibitem{Abdallaetall2023}
\reference{G. Hoerning et al}{to appear}{}{}{2023}

\bibitem{Abdollahi:2017}
\reference{Abdollahi Zadeh M, Sheykhi1 A \& Moradpour H}{\it International Journal of Modern Physics D}{\bf 26}{1750080}{2017}

\bibitem{Abdollahi:2019}
\reference{Abdollahi Zadeh M, Sheykhi1 A \& Moradpour H }{\it General Relativity and Gravitation}{\bf 51}{12}{2019}

\bibitem{Acharya:2018}\reference{Acharya B. S., Ellis S. A. R., Kane G. L., Nelson B. D. and Perry M.}{\it JHEP}{\bf 09}{130}{2018}

\bibitem{Aguilar:2022}
\reference{Aguilar-P\'erez G, Avilez-L\'opez A A and Cruz M}{\it JCAP}{\bf 11}{016}{2022}

\bibitem{Aich:2022}
\reference{Aich A}{\it Astronomy Reports }{\bf 67}{537}{2023}

\bibitem{Akaike:1974}
\reference{Akaike H}{\it IEE Trans. Autom. Control}{\bf 219}{716}{1974}

\bibitem{Akarsu:2018}
\reference{Akarsu \"O, Katirci N, Kumar S, Nunes R. C. and Sami M}{\it Physical Review D}{\bf 98}{063522}{2018}

\bibitem{Akarsu:2020}
\reference{Akarsu \"O, Katirci N, Kumar S, Nunes R. C., \"Ozt\"urk B and Sharma S}{\it The European Physical Journal C}{\bf 80}{1050}{2020}

\bibitem{Aljaf:2020}
\reference{Aljaf M, Gregoris D and  Khurshudyan M}{\it The European Physical Journal C}{\bf 80}{112}{2020}

\bibitem{Aljaf:2021}
\reference{Aljaf M, Gregoris D and  Khurshudyan M}{\it The European Physical Journal C}{\bf 81}{544}{2021}

\bibitem{Alvarez-Ortega:2022}
\reference{\'Alvarez-Ortega D, Olmo G. J., Rubiera-Garcia D, S\'aez-Chill\'on G\'omez D}{\it Physical Review D}{\bf 106}{023523}{2022}

\bibitem{1803}
\reference{Amendola Luca, Bettoni Dario, DomÃ¨nech  Guillem, Gomes Adalto R}{JCAP}{06}{029}{2018}

\bibitem{Amendola:2006kh}
\reference{L. Amendola, D. Polarski and S. Tsujikawa}{Phys. Rev. Lett}{98}{131302}{2007}

\bibitem{Amiri:2021}
\reference{Amiri H. R., Salehi A and Noroozi A. H.}{\it The European Physical Journal C}{\bf 81}{479}{2021}

\bibitem{Amon:2022}
\reference{Amon A, Gruen D, Troxel M. A. et. al.}{\it Phys. Rev. D}{\bf 105}{023514}{2022} 

\bibitem{Amon:2023}
\reference{Amon A, Roberts N. C., Miyatake H, et. al.}{\it Month. Not. Roy. Astron. Soc.}{\bf 518}{477}{2023}

\bibitem{An:2017}
\reference{An R, Feng C \& Wang B}{\it Journal of Cosmology and Astroparticle Physics}{\bf 10}{049}{2017}

\bibitem{An:2018}
\reference{An R, Feng C \& Wang B}{\it Journal of Cosmology and Astroparticle Physics}{\bf 02}{038}{2018}

\bibitem{An:2019}
\reference{An R, Xu X, Zhang J, Wang B and Yue B}{\it Journal of Cosmology and Astroparticle Physics}{\bf 01}{034}{2019}

\bibitem{An:2019b}
\reference{An R, Costa A A, Xiao L, Zhang J, and Wang B}{\it Mon. Not. Roy. Astr. Soc.}{\bf 489}{297}{2019}

\bibitem{Anchordoqui:2021}
\reference{Anchordoqui L. A., Di Valentino E, Pan S and Yang W}{\it Journal of High Energy Astrophysics}{\bf 32}{28}{2021}

\bibitem{AH2022}
\reference{Angulo R. E., Hahn O}{Liv.Rev.Comput.Astrophys.}{8}{1}{2022}

\bibitem{Annis:2022}
\referenceA{Annis J, Newman J. A. \& Slozar A}{ArXiv:2209.08049}{2022}

\bibitem{Aparicio-Resco:2021}
\reference{Aparicio Resco M and Maroto A. L.}{\it Journal of Cosmology and Astroparticle Physics}{\bf 02}{020}{2021}

\bibitem{Arevalo:2017}
\reference{Arevalo F, Cid A \& Moya J}{\it The European Physical Journal C}{\bf 77}{565}{2017}

\bibitem{Arevalo:2019}
\reference{Arevalo F, Cid A, Chimento L and Mella P}{\it The European Physical Journal C}{\bf 79}{355}{2019}

\bibitem{Asgari:2017}
\reference{Asgari M, Heymans C, Blake C,  Harnois-Deraps J, Schneider P and Van Waerbeke L}{\it Mon. Not. Roy. Astron. Soc.}{\bf 464}{1676}{2017}

\bibitem{Asghari:2019}
\reference{Asghari M, Beltr\'an Jim\'enez J, Khosravi S and Mota D F}{\it Journal of Cosmology and Astroparticle Physics}{\bf 04}{042}{2019}

\bibitem{Bachega:2020}
\reference{Bachega R. R. A., Costa A. A., Abdalla E and Fornazier K. S. F.}{\it Journal of Cosmology and Astroparticle Physics}{\bf 05}{021}{2020}

\bibitem{Bahamonde:2018}
\reference{Bahamonde S, B\"ohmer C G, Carloni S, Copeland E. J., Fang W and Tamanini N}{\it Physics Reports}{\bf 775}{1}{2018}

\bibitem{Balakin:2018}
\reference{Balakin A. B. and Ilin A. S.}{\it Symmetry }{\bf 10}{411}{2018}

\bibitem{Balakin:2021}
\reference{Balakin A. B. and Ilin A. S.}{\it Physical Review D}{\bf 105}{103525}{2021}

\bibitem{Baldi2010}
\reference{Baldi M, Pettorino V, Robbers G, Springel V}{Mon. Not. Roy. Astron. Soc.}{403}{1684--1702}{2010}

\bibitem{Baldi2011}
\reference{Baldi M}{Mon. Not. Roy. Astron. Soc.}{414}{116}{2011}

\bibitem{Baldi2012}
\reference{Baldi M}{Mon. Not. Roy. Astron. Soc.}{422}{1028--1044}{2012}

\bibitem{Baral:2021}
\reference{Baral P, Roy S. K. and Pal S}{\it Monthly Notices of the Royal Astronomical Society}{\bf 500}{2896}{2021}

\bibitem{Bautista:2017}
\reference{Bautista J E, Busca N. G., Guy J, \textit{et al.}}{Astron. Astrophys.}{\bf 603}{A12}{2017}

\bibitem{Begue:2019}
\reference{B\'egu\'e D, Stahl C and Xue S-S}{Nuclear Physics B}{\bf 904}{312}{2019}

\bibitem{Belkacemi:2020}
\reference{Belkacemi M-H, Bouabdallaoui Z, Bouhmadi-L\'opez M, Errahmani A and Ouali T}{\it International Journal of Modern Physics D}{\bf 29}{ 2050066}{2020}

\bibitem{Yang67}
\reference{Bellomo N, Bellini E, Hu B, Jimenez R, Pena- Garay C and Verde L}{JCAP}{1702}{043}{2017} 

\bibitem{Beltran:2016}
\reference{Beltr\'an Jim\'enez J., Rubiera-Garc{\'\i}a D, S\'aez-G\'omez D \& Salzano V}{\it Physical Review D} {\bf 94}{123520}{2016}

\bibitem{Beltran:2020}
\reference{Beltrán Jiménez J., Bettoni D, Figueruelo D and Teppa Pannia F. A.}{JCAP}{\bf 08}{020}{2020}

\bibitem{Beltran:2021a}
\reference{Beltr\'an Jim\'enez J, Bettoni D, Figueruelo D, Teppa Pannia F. A. and Tsujikawa S}{\it Journal of Cosmology and Astroparticle Physics}{\bf 03}{085}{2021}

\bibitem{Beltran:2021b}
\reference{Beltr\'an Jim\'enez J, Bettoni D, Figueruelo D, Teppa Pannia F. A. \& Tsujikawa S}{\it Phys. Rev. D}{\bf 104}{103503}{2021}

\bibitem{Benisty:2022}
\reference{Benisty D, Mifsud J, Levi Said J and Staicova D}{Phys. Dark Univ.}{39}{101160}{2022}

\bibitem{Bennett:2020zkv}
\reference{Bennett J. J., Buldgen G, De Salas P. F., Drewes M, Gariazzo S, Pastor S and Wong Y. Y. Y.}{JCAP}{04}{073}{2021}

\bibitem{Bernal:2016}
\reference{Bernal J. L., Verde L and Cuesta A. J.}{\it Journal of Cosmology and Astroparticle Physics}{\bf 02}{059}{2016}
 
\bibitem{Bernardi:2017}
\reference{Bernardi F. F. \& Landim R. G.}{\it The European Physical Journal C}{\bf 77}{290}{2017}

\bibitem{Bernui:2023}
\reference{Bernui A, Di Valentino E, Giar\'e W, Kumar S and Nunes R C}{Phys. Rev. D}{\bf 107}{103531}{2023}

\bibitem{Betoule:2014}
\reference{Betoule M, Kessler R, Guy J, et al}{\it Astronomy \&  Astrophysics}{\bf 568}{A22}{2014}

\bibitem{Beutler:2011}
\reference{Beutler F, et al.}{\it Mon. Not. Roy. Astron. Soc.}{\bf 416}{3017}{2011}

\bibitem{Flynn2021}
\reference{Bhandari S and Flynn C}{Universe}{\textbf{7}}{85}{2021}

\bibitem{Bhatta:2018}
\reference{Bhattacharyya A, Alam U, Pandey K. L., Das S and Pal S}{Astrophys. J.}{876}{143}{2018}

\bibitem{Biswas:2021}
\reference{Biswas S. K. and Biswas A}{\it European Physical Journal C}{\bf 81}{356}{2021}

\bibitem{Blanchard:2021}
\reference{Blanchard A and Ili\'c S}{Astron. Astrophys.}{656}{A75}{2021}

\bibitem{Yang82}
\reference{Boehmer C. G., Tamanini N and Wright M}{Phys. Rev. D}{91}{123002}{2015}

\bibitem{Yang83}
\reference{Boehmer C. G., Tamanini N and Wright M}{Phys. Rev. D}{91}{123003}{2015}

\bibitem{Yang76}
\reference{Bonilla A, Nunes R. C. and Abreu E. M. C.}{Mon. Not. Roy. Astron. Soc.}{485}{2486}{2019}

\bibitem{Bonilla:2022}
\reference{Bonilla A, Kumar S, Nunes R C and Pan S}{\it Monthly Notices of the Royal Astronomical Society}{\bf 512}{4231}{2022}

\bibitem{Bouhmadi:2018}
\reference{Bouhmadi-L\'opez M, Errahmani A, Ouali T and Tavakoli Y}{\it The European Physical Journal C}{\bf 78}{330}{2018}

\bibitem{BoussoPolchinski2000}
\reference{R. Bousso and J. Polchinski}{ JHEP}{ 06}{006}{2000} 

\bibitem{Bowman:2018}
\reference{Bowman J. D., Rogers A. E. E., Monsalve R A, Mozdzen T J and Mahesh N}{\it Nature}{\bf 555}{67}{2018}

\bibitem{Yang84}
\reference{Bruck C van de and Morrice J}{JCAP}{1504}{036}{2015} 

\bibitem{Bruck:2018}
\reference{Bruck C van de and Mifsud J}{\it Phys. Rev. D}{\bf 97}{023506}{2018} 

\bibitem{Bruck:2020}
\reference{Bruck C van de and Teixeira E M}{\it Phys. Rev. D}{\bf 102}{103503}{2020} 

\bibitem{Bull:2015}
\reference{Bull P, Ferreira P. G., Patel P \& Santos M. G.}{\it The Astrophysical Journal}{\bf 803}{21}{2015}

\bibitem{Cai:2017}
\reference{Cai R-G, Tamanini N and Yang T}{\it Journal of Cosmology and Astroparticle Physics}{\bf 05}{031}{2017}

\bibitem{Califano:2023}
\reference{Califano M, de Martino I, Vernieri D and Capozziello S}{\it Monthly Notices of the Royal Astronomical Society}{\bf 518}{3372}{2023}

\bibitem{Califano:2023b}
\reference{Califano M, de Martino I, Vernieri D and Capozziello S}{\it Phys. Rev. D}{\bf 107}{123519}{2023}

\bibitem{Capozziello:2011et}
\reference{S. Capozziello and M. De Laurentis, Mariafelicia}{Phys. Rept}{509}{167}{2011}

\bibitem{Caprini:2016}
\reference{Caprini C \& Tamanini N}{\it Journal of Cosmology and Astroparticle Physics}{\bf 10}{006}{2016}

\bibitem{Cardenas:2020}
\reference{C\'ardenas V. H. and Lepe S}{\it The European Physical Journal C}{\bf 80}{862}{2020}

\bibitem{Cardona:2022}
\reference{Cardona W \& Figueruelo D}{\it Journal of Cosmology and Astroparticle Physics}{\bf 12}{010}{2022}

\bibitem{Carlesi2014a}
\reference{Carlesi E, Knebe A, Lewis G, Wales S, Yepes G}{Mon. Not. Roy. Astron. Soc.}{439}{2943--2957}{2014}

\bibitem{Carlesi2014b}
\reference{Carlesi E, Knebe A, Lewis G, Yepes G}{Mon. Not. Roy. Astron. Soc.}{439}{2958--2969}{2014}

\bibitem{Chagoya:2023}
\reference{Chagoya J, L\'opez-Domnguez J C and Ortiz C}{Classical and Quantum Gravity}{40}{075005}{2023}

\bibitem{Saikat2021}
\reference{Chakraborty S, Gonz\'alez E, Leon G and Wang B}{Eur. Phys. J. C}{81}{1039}{2021}

\bibitem{Chamings:2020}
\reference{Chamings F N, Avgoustidis A, Copeland E J, Green A M and Pourtsidou A}{\it Phys. Rev.
D}{\bf 101}{043531}{2020}

%\bibitem{chen1}
%\reference{S.~B.~Chen, B.~Wang, J.~L.~Jing}{Phys.Rev. D}{78}{123503}{2008}

%\bibitem{chen2}
%\reference{X.~M.~Chen, B.~Wang, N.~Pan, Y.~G.~Gong}{Phys.Lett. B}{695}{30}{2011}

\bibitem{Cheng:2020}
\reference{Cheng G, Ma Y-Z, Wu F, Zhang J and Chen X}{\it Physical Review D}{\bf 102}{043517}{2020}

\bibitem{Yang72}
\reference{Choudhury S. R and Choubey S}{JCAP}{\bf 1809}{017}{2018} 

\bibitem{Yang73}
\reference{Choudhury S. R. and Hannestad S}{JCAP}{\textbf{07}}{037}{2020}

\bibitem{Chibana:2019}
\reference{Chibana F, Kimura R, Yamaguchi M, Yamauchi D and Yokoyama S}{\it JCAP}{\bf 10}{049}{2019}

\bibitem{Chimento:2003}
\reference{ Chimento L P, Jakubi A S, Pav\'on D and Zimdahl W}{Physical Review D}{\textbf{67}}{083513}{2003}

\bibitem{Boehmer:2015kta}
\reference{G. Christian, N. Tamanini and M. Wright, Matthew}{Phys. Rev. D}{91}{123002}{2015}

\bibitem{Cicoli:2023opf}
\referenceA{Michele Cicoli, Joseph P. Conlon, Anshuman Maharana, Susha Parameswaran, Fernando Quevedo and Ivonne Zavala}{arXiv:2303.04819}{2023}

\bibitem{Cid:2019}
\reference{Cid A, Santos B, Pigozzo C, Ferreira T and Alcaniz J}{\it Journal of Cosmology and Astroparticle Physics}{\bf 03}{030}{2019}

\bibitem{Colpi:2016fup}
\referenceA{Colpi Monica and Sesana Alberto}{arXiv:1610.05309}{2016}

\bibitem{Costa:2017}
\reference{Costa A. A., Xu X-D, Wang B \& Abdalla E}{\it Journal of Cosmology and Astroparticle Physics}{\bf 01}{028}{2017}

\bibitem{Costa:2018}
\reference{Costa A. A., Landim R. C. G., Wang B \& Abdalla E}{\it The European Physical Journal C}{\bf 78}{746}{2018}

\bibitem{Costa:2019}
\reference{Costa A. A., Marcondes R. J. F., Landim R. C. G., et al}{\it Monthly Notices of the Royal Astronomical Society}{\bf 488}{78}{2019}

\bibitem{Costa2021}
\reference{Costa A. A., et al.}{Astron. Astrophys.}{664}{A20}{2022}

\bibitem{Crocce2006}
\reference{Crocce M, Pueblas S, Scoccimarro R}{Mon. Not. Roy. Astron. Soc.}{373}{369--381}{2006}

\bibitem{Cruz:2018}
\reference{Cruz M and Lepe S}{\it Classical and Quantum Gravity}{\bf 15}{155013}{2018}

\bibitem{Cruz:2019}
\reference{Cruz M, Lepe S and Morales-Navarrete G}{\it Nuclear Physics B}{\bf 943}{114623}{2019}

\bibitem{Cruz:2020}
\reference{Cruz M and Lepe S}{\it Nuclear Physics B}{\bf 956}{115017}{2020}

\bibitem{Dam:2019}
\reference{Dam L, Bolejko K and Lewis G F}{\it JCAP}{\bf 12}{030}{2019}

\bibitem{Kaplor2016}
\reference{D'Amico G, Hamill T and Kaloper N}{Phys. Rev. D}{94}{103526}{2016}

\bibitem{DeArcia:2023}
\reference{De Arcia R, Quir\'os I, Nucamendi U and Gonz\'alez T}{\it Physics of the Dark Universe}{\bf 40}{101183}{2023}

\bibitem{deCesare:2022}
\reference{de Cesare M and Wilson-Ewing E}{\it Phys. Rev. D}{\bf 106}{023527}{2022}

\bibitem{DeFelice:2010aj}
\reference{De Felice A and Tsujikawa S}{Living Rev. Rel.}{13}{3}{2010}

\bibitem{deMartino:2018}
\reference{de Martino I}{\it Symmetry}{\bf 10}{372}{2018}

\bibitem{Deogharia:2021}
\reference{Deogharia G, Bandyopadhyay M and Biswas R}{\it Modern Physics Letters A}{\bf 36}{2150275}{2021}

\bibitem{Des:2023}
\referencelink{https://www.darkenergysurvey.org/}

\bibitem{deSa:2022}
\reference{de S\'a R, Benetti M and Graef L}{\it The European Physical Journal Plus}{\bf 137}{1129}{2022}

\bibitem{Dhawan:2022}
\reference{Dhawan S, Goobar A, Johansson J, et al}{\it The Astrophysical Journal} {\bf 934}{185}{2022}

\bibitem{Dimopoulos2008}
\reference{Dimopoulos S, Kachru S, McGreevy J and Wacker J. G.}{JCAP}{08}{003}{2008}

\bibitem{DiValentino:2017}
\reference{Di Valentino E, Melchiorri A \& Mena O}{\it Physical Review D}{\bf 96}{043503}{2017}

\bibitem{DiValentino:2020a}
\reference{Di Valentino E, Melchiorri A, Mena O and Vagnozzi S}{\it Physics of the Dark Universe}{\bf 30}{100666}{2020}

\bibitem{DiValentino:2020b}
\reference{Di Valentino E, Melchiorri A, Mena O and Vagnozzi S}{\it Physical Rev D}{\bf 101}{063502}{2020}

\bibitem{DiValentino:2020c}
\reference{Di Valentino E, Gariazzo S, Mena O and Vagnozzi}{\it Journal of Cosmology and Astroparticle Physics}{\bf 07}{045}{2020}

\bibitem{DiValentino:2021a}
\reference{Di Valentino E, Melchiorri A and Silk J}{\it The Astrophysical Journal Letters}{\bf 908}{L9}{2021}

\bibitem{DiValentino:2021b}
\reference{Di Valentino E, Mena O, Pan S, Visinelli L, Yang W Melchiorri A, Mota D. F., Riess A. G. and Silk J}{\it Classical and Quantum Gravity}{\bf 38}{ 153001}{2021}

\bibitem{DiValentino:2021hoh}
\reference{Di Valentino E, Gariazzo S and Mena O}{Phys. Rev. D}{104}{083504}{2021}

\bibitem{DiValentino:2021c}
\reference{Di Valentino E, Melchiorri A, Mena O, Pan S and Yang W}{\it Monthly Notices of the Royal Astronomical Society}{\bf 502}{L23}{2021}

\bibitem{DiValentino:2021d}
\reference{Di Valentino E}{\it Monthly Notices of the Royal Astronomical Society}{\bf 502}{2065}{2021}

\bibitem{Dixit:2020}
\reference{Dixit A, Bhardwaj V. K. and Pradhan A}{\it The European Physical Journal Plus}{\bf 135}{10}{2020}

\bibitem{DuffandBibber}
\reference{ Leanne D Duffy and Karl van Bibber }{New Journal of Physics}{ 11}{ }{ 2009}

\bibitem{duMas:2017}
\reference{du Mas des Bourboux H, Le Goff J. M., et al.}{Astron. Astrophys.}{\bf 608}{A130}{2017}

\bibitem{Duniya:2022a}
\referenceA{Duniya D. G. A.}{ArXiv:2203.12582}{2022}

\bibitem{Duniya:2022b}
\reference{Duniya D. G. A. and Kumwenda M}{\it Monthly Notices of the Royal Astronomical Society}{\bf 522}{3308}{2022}

\bibitem{Dusoye:2021}
\reference{Dusoye A, de la Cruz-Dombriz A, Dunsby P and Nunes N J}{\it JCAP}{\bf 03}{002}{2021}

\bibitem{Dusoye:2023}
\reference{Dusoye A, de la Cruz-Dombriz A, Dunsby P and Nunes N J}{\it JCAP}{\bf 01}{001}{2023}

\bibitem{Dutta:2018}
\reference{Dutta J, Khyllep W and Saridakis E N}{\it JCAP}{\bf 02}{041}{2018}

%\bibitem{duran3}
%\reference{I.~Dur\'an, F.~Atrio-Barandela, D.~Pav\'on}{JCAP}{04}{008}{2012}

\bibitem{Escamilla-Rivera:2021}
\reference{Escamilla-Rivera C and Gamboa A}{\it The European Physical Journal Plus}{\bf 137}{254}{2021}

\bibitem{Euclid:2023}
\referencelink{https://www.euclid-ec.org/}

\bibitem{Faraoni:2021}
\reference{Faraoni V, Jose S and Dussault S}{\it General Relativity and Gravitation}{\bf 53}{109}{2021}

%\bibitem{feng1}
%\reference{C.~Feng, B.~Wang, Y.~G.~Gong, R.-K.~Su}{JCAP}{0709}{005}{2007}

\bibitem{Feng:2016}
\reference{Feng L \& Zhang X}{\it Journal of Cosmology and Astroparticle Physics}{\bf 08}{072}{2016}

\bibitem{Feng:2018}
\reference{Feng L, Li Y-H, Yu F, Zhang J-F and Zhang X}{\it The European Physical Journal C}{\bf 78}{865}{2018}

\bibitem{Froustey:2020mcq}
\reference{Froustey J, Pitrou C and Volpe M. C.}{JCAP}{12}{015}{2020}

\bibitem{Yang80}
\reference{Feng L, Zhang J. F. and Zhang X}{Phys. Dark Univ.}{23}{100261}{2019}

%\bibitem{Yang78}
%\reference{L. Feng, H. L. Li, J. F. Zhang and X. Zhang}{Sci. China Phys. Mech. Astron.}{63}{220401}{2020} 

\bibitem{Feng:2020a}
\reference{Feng L, Li H-L, Zhan J-F and Zhang X}{\it Science China Physics, Mechanics \& Astronomy}{\bf 63}{220401}{2020}

\bibitem{Feng:2020b}
\reference{Feng L, Li H-L, Zhan J-F and Zhang X}{\it Science China Physics, Mechanics \& Astronomy}{\bf 63}{290404}{2020}

%\bibitem{feng2}
%\reference{C.~Feng, B.~Wang, E.~Abdalla, R.-K.~Su}{Phys.Lett. B}{665}{111}{2008}

\bibitem{Ferramacho:2013}
\reference{Ferramacho L D, Blanchard A and Zolnierowski Y}{Astron. Astrophys.}{\bf 499}{21}{2009}

\bibitem{Figueruelo:2021}
\reference{Figueruelo D, Aparicio Resco M, \textit{et al.}}{\it JCAP}{\bf 07}{022}{2021}

\bibitem{Font-Ribera:2014}
\reference{Font-Ribera A et al}{\it Journal of Cosmology and Astroparticle Physics}{\bf 05}{027}{2014}
 
\bibitem{Fornazier2021}
\reference{Fornazier K. S. F., et al.}{Astron. Astrophys.}{664}{A18}{2022}

\bibitem{FW2012}
\reference{Frenk C. S., White S. D. M.}{Annalen Phys.}{524}{507--534}{2012}

\bibitem{Galvany:2022}
\reference{Galbany L, de Jaeger T, Riess A, et al}{\it Astron.Astrophys.}{\bf 679}{A95}{2023}

\bibitem{Gao2014}
\reference{Gao H, Li Z and Zhang B}{Astrophys. J.}{\textbf{788}}{189}{2014}

\bibitem{Gariazzo:2022}
\reference{Gariazzo S, Di Valentino E, Mena O and Nunes R. C.}{\it Physical Review D}{\bf 106}{023530}{2022}

\bibitem{Kumar22}
\reference{Geng C. Q., Lee C. C., Shen J. L.}{Phys. Lett. B}{740}{285}{2015}

\bibitem{Yang65}
\reference{Gerbino M, Freese K, Vagnozzi S, Lattanzi M, Mena O, Giusarma E and Ho S}{Phys. Rev. D}{95}{043512}{2017} 

\bibitem{Ghaffari:2018}
\reference{Ghaffari S, Moradpour H, Lobo I P, Gra{\c{c}}a J. P. M. and Bezerra V. B.}{\it The European Physical Journal C} {\bf 78}{706}{2018}

\bibitem{Ghodsi:2023}
\reference{Ghodsi Yengejeh M, Fakhry S, Firouzjaee J T and Fathi H}{\it Physics of the Dark Universe} {\bf 39}{101144}{2023}

\bibitem{Gil-Marin:2016}
\reference{Gil-Mar{\'\i}n H, et al.}{\it Mon. Not. Roy. Astron. Soc.}{\bf 460}{4210}{2016}

\bibitem{Schutz2002}
\referenceB{Gilfanov M, Sunyaev R and Churazov E}{In lighthouses of the Universe}{Springer}{2002}

\bibitem{Yang64}
\reference{Giusarma E, Gerbino M, Mena O, Vagnozzi S, Ho S and Freese K}{Phys. Rev. D}{94}{083522}{2016}

\bibitem{Yang81}
\reference{Gleyzes J, Langlois D, Mancarella M and Vernizzi F}{JCAP}{1508}{054}{2015}

\bibitem{Gomez:2023}
\reference{G\'omez G }{\it Phys. Rev. D}{\bf 107}{123535}{2023}

\bibitem{Gong2021}
\reference{Gong Yungui, Luo Jun, Wang Bin}{Nature Astronomy}{\textbf{5}}{881-889}{2021}

\bibitem{Grandon:2019}
\reference{Grandon D and Cardenas V H}{Gen.Rel.Grav.}{\textbf{51}}{42}{2019}

\bibitem{Guo:2017}
\reference{Guo R-Y, Li Y-H, Zhang J-F \& Zhang X}{\it Journal of Cosmology and Astroparticle Physics}{\bf 05}{040}{2017}

\bibitem{Yang79}
\reference{Guo R. Y., Zhang J. F. and Zhang X}{\it Chin. Phys. C}{42}{095103}{2018} 

\bibitem{Guo:2018a}
\reference{Guo J-J, Zhang J-F, Li Y-H and Zhang X}{\it Science China Physics, Mechanics \& Astronomy}{\bf 3}{30011}{2018}

\bibitem{Guo:2021}
\reference{Guo R-Y, Feng L, Yao T-Y and Chen X-Y}{\it Journal of Cosmology and Astroparticle Physics}{\bf 12}{036}{2021}

\bibitem{Guy:2023}
\reference{Guy J, Bailey S, Kremin A et al}{\it Astronomical Journal}{\bf 165}{144}{2023}

\bibitem{Halder:2021}
\reference{Halder A and Pandey M}{\it Monthly Notices of the Royal Astronomical Society}{\bf 508}{3446}{2021}

\bibitem{Hall2012}
\reference{Hall A, Bonvin C, Challinor A}{Phys. Rev. D}{87}{064026}{2013}

\bibitem{Hanany:2019}
\referenceA{Hanany S, Alvarez M, Artis E et al}{ArXiv:1902.10541}{2019}

\bibitem{Harko:2022}
\reference{Harko T, Asadi K, Moshafi H and Sheikhahmadi H}{\it Physics of the Dark Universe}{\bf 38}{101131}{2022}

%\bibitem{he1}
%\reference{J.~H.~He, B.~Wang}{JCAP}{0806}{010}{2008}

\bibitem{He2013}
\reference{He Jian-hua}{Phys. Rev. D}{88}{103523}{2013}

\bibitem{he2}
\reference{He J. H., Wang B, Abdalla E}{Phys.Lett. B}{671}{139}{2009}

\bibitem{He:2011qn}
\reference{J. He, B. Wang and E. Abdalla}{Phys. Rev. D}{84}{123526}{2011}

%\bibitem{he3}
%\reference{J.~H.~He, B.~Wang, Y.~P.~Jing}{JCAP}{0907}{030}{2009}

%\bibitem{he4}
%\reference{J.~H.~He, B.~Wang, P.~J.~Zhang}{Phys.Rev. D}{80}{063530}{2009}

%\bibitem{he5}
%\reference{J.~H.~He, B.~Wang}{AIP Conf.Proc.}{1122}{292}{2009}

%\bibitem{he6}
%\reference{J.~H.~He, B.~Wang, E.~Abdalla, D.~Pavon}{JCAP}{1012}{022}{2010}

%\bibitem{he7}
%\reference{J.~H.~He, B.~Wang}{J.Phys.Conf.Ser.}{222}{012029}{2010}

%\bibitem{he8}
%\reference{J.~H.~He, B.~Wang, E.~Abdalla}{Phys.Rev. D}{83}{063515}{2011}

%\bibitem{he9}
%\reference{J.~H.~He, B.~Wang, E.~Abdalla}{Phys.Rev. D}{84}{123526}{2011}

\bibitem{Heymans:2013}
\reference{Heymans C, Grocutt E, \textit{et al.}}{\it Mon. Not. Roy. Astron. Soc.}{\bf 432}{2433}{2013}

\bibitem{Hikage:2019}
\reference{Hikage C, Oguri M, Hamana T et al.}{\it Pub. Astron.  Soc. Japan}{\bf 71}{43}{2019}

\bibitem{Hildebrandt:2017}
\reference{Hildebrandt H, Viola M, \textit{et al.}} {\it Mon. Not. Roy. Astron. Soc.}{\bf 465}{1454}{2017}

\bibitem{Hildebrandt:2020}
\reference{Hildebrandt H, K\"ohlinger F, van den Busch J. L.
et al}{\it Astron. \& Astrophys.}{\bf 633}{69}{2020}  

\bibitem{Honecker:2016}
\reference{Gabriele Honecker}{\it Int. J. Mod. Phys. }{\bf A 31}{1630050}{2016} 

\bibitem{2211}
\reference{Hou Wan-Ting, Qi Jing-Zhao, Han Tao, Zhang Jing-Fei, Cao Shuo, Zhang Xin}{\it JCAP}{\bf 05}{017}{2023}

\bibitem{Hu1998}
\reference{Hu W, Eisenstein D. J. and Tegmark M}{Phys. Rev. Lett.}{80}{5255}{1998}

\bibitem{Hughes2002}
\reference{Hughes S. A.}{Mon. Not. Roy. Astron. Soc.}{\textbf{331}}{805}{2002}

\bibitem{Huterer:2018}
\reference{Huterer D and Shafer D. L.}{\it Reports on Progress in Physics}{\bf 81}{6901}{2018}

\bibitem{Izaurieta:2020}
\reference{Izaurieta F and Lepe S}{\it Classical and Quantum Gravity}{\bf 37}{205004}{2020}

\bibitem{Izquierdo:2018}
\reference{Izquierdo G, Blanquet-Jaramillo R. C. and Sussman R. A.}{\it The European Physical Journal C}{\bf 78}{223}{2018}

\bibitem{Johnson:2021a}
\reference{Johnson J. P. and Shankaranarayanan S}{\it Physical Review D}{\bf 103}{023510}{2021}

\bibitem{Johnson:2021b}
\reference{Johnson J. P., Sangwan A and Shankaranarayanan S}{\it Journal of Cosmology and Astroparticle Physics}{\bf 01}{024}{2021}

\bibitem{Joseph:2023}
\reference{Joseph A and Saha R}{Monthly Notices of the Royal Astronomical Society}{\bf 519}{1809}{2023}

\bibitem{Jpas:2023}
\referencelink{https://www.j-pas.org/}

\bibitem{Karwan:2017}
\reference{Karwan K and Sapa S}{\it The European Journal of Physics C}{\bf 77}{352}{2017}

\bibitem{Kase:2020}
\reference{Kase R and Tsujikawa S}{\it Phys. Rev. D}{\bf 101}{063511}{2020}

\bibitem{Kashlinsky:2015}
\reference{Kashlinsky A, Arendt R, Atrio-Barandela F \& Helgason K }{\it The Astrophysical Journal}{\bf 813}{L12}{2015}

\bibitem{Kashlinsky:2018}
\reference{Kashlinsky A, Arendt R, Atrio-Barandela F, Cappelluti N, Ferrara A \& Hasinger G}{\it Rev. Mod. Phys.}{\bf 90}{025006}{2018}

\bibitem{Khlinger:2017}
\reference{K\"ohlinger F, Viola M, \textit{et al.}}{\it Mon. Not. Roy. Astron. Soc.}{\bf 471}{4412}{2017}

\bibitem{Khyllep:2021}
\reference{Khyllep W, Dutta J, Basilakos S and Saridakis E. N.}{\it Physical Review D}{\bf 105}{043511}{2021}

\bibitem{Koivistoetall2014}
\reference{T. Koivisto, D. Wills, I. Zavala}{JCAP}{ 06} {036}{2014}

\bibitem{Komatsu2011}
\reference{Komatsu E et al.}{ Astrophys. J. Suppl.}{192}{18}{2011} 

\bibitem{Kumar:2016}
\reference{Kumar S \& Nunes R. C.}{\it Physical Review D}{\bf 94}{123511}{2016}

\bibitem{Kumar:2017a}
\reference{Kumar S \& Nunes R. C.}{\it The European Physical Journal C}{\bf 77}{734}{2017}

\bibitem{Kumar:2017b}
\reference{Kumar S \& Nunes R. C.}{\it Physical Review D}{\bf 96}{103511}{2017}

\bibitem{Kumar:2019}
\reference{Kumar S, Nunes R. C. and Yadav S. K.}{\it The European Physical Journal C}{\bf 79 }{576}{2019}


\bibitem{Linder2019}
\reference{Kumar Pawan, Linder Eric V}{Phys. Rev. D}{100}{083533}{2019}

\bibitem{Kumar:2021}
\reference{Kumar S}{\it Physics of the Dark Universe}{\bf 33}{100862}{2021}

\bibitem{LandimBernardiAbdalla}\reference{R. G. Landim, R. Marcondes, F. Bernardi and E. Abdalla}{\it Braz. J. Phys.}{\bf 48}{364}{2018}. 

\bibitem{Landim:2016isc}
\reference{R. G. Landim and E. Abdalla}{Phys. Lett. B}{764}{271}{2017}

\bibitem{Landim:2022}
\reference{Landim R}{\it Physical Review D}{\bf 106}{043527}{2022}

\bibitem{Yang63}
\reference{Lattanzi M and Gerbino M}{Front. in Phys.}{5}{70}{2018}

\bibitem{Yang85}
\reference{La Vacca G, Kristiansen J. R., Colombo L. P. L., Mainini R and Bonometto S. A.}{JCAP}{0904}{007}{2009}

\bibitem{Lepe:2016}
\reference{Lepe S and Pe\~na F}{\it The European Physical Journal C}{\bf 76}{507}{2016}

\bibitem{Yang62}
\reference{Lesgourgues J and Pastor S}{Phys. Rept.}{429}{307}{2006}

\bibitem{Li:2019}
\reference{Li C and Cai Y-F}{\it Physics Letters B}{\bf 788}{70}{2019}

\bibitem{Huillier2017}
\reference{L'Huillier B, Winther H, Mota D, Park C, Kim J}{Mon. Not. Roy. Astron. Soc.}{468}{3174--3183}{2017}

\bibitem{LiC:2020}
\reference{Li C, Ren X, Khurshudyan and Cai Y-F}{\it Physics Letters B}{\bf 801}{135141}{2020}

\bibitem{Li:2020}
\reference{Li H, Yang W and Wu Y}{\it Physics of the Dark Universe}{\bf 20}{78}{2017}

\bibitem{LiH-L:2020}
\reference{Li H-L, Zhang J-F and Zhang X}{\it Communications in Theoretical Physics}{\bf 72}{125401}{2020}

\bibitem{Liao2018}
\reference{Liao S}{Mon. Not. Roy. Astron. Soc.}{481}{3750--3760}{2018}

\bibitem{Liccardo2021}
\reference{Liccardo V, et al.}{Astron. Astrophys.}{664}{A17}{2022}

\bibitem{Linton:2022}
\reference{Linton M. S., Crittenden R \& Pourtsidou A}{\it Journal of Cosmology and Astroparticle Physics}{\bf 08}{75}{2022}

\bibitem{LiteBird:2023}
\referencelink{https://www.isas.jaxa.jp/en/missions/spacecraft/future/litebird.html}

\bibitem{LiuG:2023}
\reference{Liu G, Zhou Z, Mu Y and Xu L}{\it Phys. Rev. D }{\bf 108}{083523}{2023}

\bibitem{Liu:2021}
\reference{Liu Y,  Liao S, Liu X, Zhang J, An R and Fan Z}{\it Monthly Notices of the Royal Astronomical Society}{\bf 511}{3076}{2021}

\bibitem{Liu2022}
\reference{Liu Y, Liao S, Liu X, Zhang J, An R, Fan Z}{Mon. Not. Roy. Astron. Soc.}{511}{3076--3088}{2022}

\bibitem{Kumar23}
\reference{Lu J, Liu M, Wu Y, Wang Y and Yang W}{Eur. Phys. J. C}{\textbf{76}}{679}{2016} 

\bibitem{Lucca:2020}
\reference{Lucca M and Hooper D C}{\it Physical Review D}{\bf 102}{123502}{2020}

\bibitem{Lucca:2021}
\reference{Lucca M}{\it Physics of the Dark Universe}{\bf 34}{100899}{2021}

\bibitem{Ludwick:2021}
\reference{Ludwick K. J. and Sebaugh H}{\it Modern Physics Letters A}{\bf 36}{2150122}{2021}

\bibitem{Mandal:2023}
\reference{Mandal G, Chakraborty S, Mishra S and Biswas S K}{\it Physics of the Dark Universe }{\bf 40}{101210}{2023}

\bibitem{Marsh:2015xka}
\reference{D. J. E. Marsh}{Phys. Rept}{643}{1}{2016}

\bibitem{Marcondes:2016}
\reference{Marcondes R. J. F., Landim R. C. G., Costa A. A., Wang B \& Abdalla E}{\it Journal of Cosmology and Astroparticle Physics}{\bf 12}{009}{2016}

\bibitem{Mawas:2021}
\referenceA{Mawas E, Street L, Gass R and Wijewardhana L. C. R.}{ArXiv:2108.13317}{2021}

\bibitem{Micheletti:2009pk}
\reference{S.~Micheletti, E.~Abdalla, B.~Wang}{Phys.Rev. D}{79}{123506}{2009}

\bibitem{1901}
\reference{Mifsud Jurgen, van de Bruck Carsten}{\it Monthly Notices of the Royal Astronomical Society}{\bf 487}{900}{2019}

\bibitem{Mifsud:2017}
\reference{Mifsud Jurgen, van de Bruck Carsten}{\it JCAP}{\bf 11}{001}{2017}

\bibitem{Minoda:2023}
\reference{Minoda T, Saga S, Takahashi T, Tashiro H, Yamauchi D, Yokoyama S \& Yashiura S}{\it Publications of the Astronomical Society of Japan}{\bf 75}{S154}{2023}

\bibitem{Mishra:2023}
\reference{Mishra K R, Pacif S K J and Kumar R}{Physics of the Dark Universe}{\bf 40}{101211}{2023}

\bibitem{Moresco:2016}
\reference{Moresco M et al}{\it JCAP}{\bf 1605}{014}{2016}

\bibitem{Mortsell:2021}
\reference{Mortsell E, Goobar A, Johansson J and Dhawan S}{Astrophys. J.}{933}{212}{2022}

\bibitem{Mukherjee:2016}
\reference{Mukherjee A}{\it Journal of Cosmology and Astroparticle Physics}{\bf 11}{ 055}{ 2016}

\bibitem{Mukherjee:2021}
\reference{Mukherjee P and Banerjee N}{\it Physical Review D}{\bf 103}{123530}{2021}

\bibitem{Mukherjee:2022}
\reference{Mukherjee P and Banerjee N}{\it Physics of the Dark Universe}{\bf 36}{100998}{2022}

\bibitem{Mukhopadhyay:2021}
\reference{Mukhopadhyay U, Majumdar D and Datta K. K.}{\it Physical Review D}{\bf 103}{063510}{2021}

\bibitem{Nakamura:2019}
\reference{Nakamura S, Kase R and Tsujikawa S}{\it JCAP}{\bf 12}{023}{2019}

\bibitem{Nayak:2020}
\reference{Nayak B}{\it Gravitation and Cosmology}{\bf 26}{273}{2020}

\bibitem{Nojiri:2006je}\reference{S. Nojiri, S. Odintsov and M. Sami}{Phys. Rev. D}{74}{046004}{2006}

\bibitem{Nunes:2016}
\reference{Nunes R. C., Pan S \& Saridakis E. N.}{\it Physical Review D}{\bf 94}{023508}{2016}

\bibitem{Yang68}
\reference{Nunes R. C. and Bonilla A}{Mon. Not. Roy. Astron. Soc.}{473}{4404}{2018}

\bibitem{Nunes:2022}
\reference{Nunes R. C., Vagnozzi S, Kumar S, Di Valentino E and Mena O}{\it Physical Review D}{\bf 105}{123506}{2022}

%\bibitem{olivares1}
%\reference{G.~Olivares, F.~Atrio-Barandela, D.~Pav\'on}{Phys. Rev. D.}{71}{063523}{2005}

%\bibitem{olivares2}
%\reference{G.~Olivares, F.~Atrio-Barandela, D.~Pav\'on}{Phys. Rev. D.}{74}{043521}{2006}

%\bibitem{olivares3}
%\reference{G.~Olivares, F.~Atrio-Barandela, D.~Pav\'on}{Phys. Rev. D.}{77}{063513}{2008}

%\bibitem{olivares4}
%\reference{G.~Olivares, F.~Atrio-Barandela, D.~Pav\'on}{Phys. Rev. D.}{77}{103520}{2008}

\bibitem{Ong2023} 
\reference{Ong Y C}{\it Universe}{\bf 9}{437}{2023}

\bibitem{OoguriPaltiShiuVafa2019} 
\reference{ H. Ooguri, E. Palti, G. Shiu, and C. Vafa}{Phys. Lett. B}{788}{180}{2019}

\bibitem{Otalora:2022}
\reference{Otalora G and Saridakis E. N.}{\it Physics Letters B}{\bf 842}{137970}{2023}

\bibitem{Paliathanasis:2019}
\reference{Paliathanasis A, Pan S and Yang W}{\it International Journal of Modern Physics D}{\bf 28}{1950161}{2019}

\bibitem{Palma:2023}
\reference{Palma D and Candlish G N}{\it Month. Not. Roy. Astron. Soc. }{\bf 526}{1904}{2023}

\bibitem{Palti:2019pca}
\reference{E. Palti}{Fortsch. Phys}{67}{1900037}{2019}

\bibitem{Pan:2017}
\reference{Pan S and Sharov G. S.}{\it Monthly Notices of the Royal Astronomical Society}{\bf 472}{4736}{2017}

\bibitem{Pan:2018}
\reference{Pan S, Mukherjee A and Banerjee N}{\it Monthly Notices of the Royal Astronomical Society}{\bf 477}{1189}{2018}

\bibitem{Pan:2019a}
\reference{Pan S, Yang W, Di Valentino E, Saridakis E. N. and Chakraborty S}{\it Physical Review D}{\bf 100}{103520}{2019}

\bibitem{Pan:2020a}
\reference{Pan S, Yang W and Paliathanasis A}{\it  Monthly Notices of the Royal Astronomical Society}{\bf 493}{3114}{2020}

\bibitem{Pan:2019b}
\reference{Pan S, Yang W, Singha C and Saridakis E N}{\it Physical Review D}{\bf 100}{083539}{2019}

\bibitem{Pan:2020b}
\reference{Pan S, Sharov G. A. and Yang W}{\it Physical Review D}{\bf 101}{103533}{2020}

\bibitem{Pan:2020c}
\reference{Pan S, de Haro J, Yang W and Amor\'os J}{\it Physical Review D}{\bf 101}{123506}{2020}

\bibitem{Panotopoulos:2020}
\reference{Panotopoulos G, Rinc\'on A, Otalora G and Videla N}{\it The European Physical Journal C}{\bf 80}{286}{2020}

\bibitem{Patil:2023}
\reference{Patil T and Panda S}{\it The European Physical Journal Plus}{\bf 138}{583}{2023}

%\bibitem{pavon1}
%\reference{D.~Pavon, B.~Wang}{Gen.Rel.Grav.}{41}{1}{2009}

\bibitem{Penzo2016}
\reference{Penzo C, Macciò A. V., Baldi M, Casarini L, Oñorbe J}{Mon. Not. Roy. Astron. Soc.}{461}{2490--2501}{2016}

\bibitem{Perivolaropoulos:2022}
\reference{Perivolaropoulos L and Skara F}{\it New Astronomy Reviews}{\bf 95}{101659}{2022}

\bibitem{Platts2018}
\reference{Petroff E, Hessels J. W. T., Lorimer D. R.}{Astron. Astrophys. Rev.}{30}{2}{2022}

\bibitem{Planck:2014}
\reference{Planck Collaboration}{\it Astron. Astrophys.}{\bf 571}{A16}{2014}


\bibitem{Planck:2016}
\reference{Planck Collaboration}{\it Astron. Astrophys.}{\bf 594}{A24}{2016}

\bibitem{Planck_2018_1:2020}
\reference{Planck Collaboration}{\it Astron. Astrophys.}{\bf 641}{A1}{2020}

\bibitem{Planck_2018_5:2020}
\reference{Planck Collaboration}{\it A\& A}{\bf 641}{A5}{2020}

\bibitem{Planck_2018_6:2020}
\reference{Planck Collaboration}{\it Astron. Astrophys.}{\bf 641}{A6}{2020}

\bibitem{Starobinsky1992}
\reference{Polarski D and Starobinsky A. A.}{Nucl. Phys. B}{385}{623-650}{1992}

\bibitem{Poulin:2018}
\reference{Poulin V, Boddy K. K., Bird S and Kamionkowski M}{Phys. Rev. D.}{97}{123504}{2018}

\bibitem{Pourtsidou:2016}
\reference{Pourtsidou A and Tram T}{\it Phys. Rev. D}{\it 94}{ 043518}{2016}

\bibitem{Pradhan:2020}
\reference{Pradhan A, Goswami G. K., Beesham A and Dixit A}{\it New Astronomy}{\bf 78}{101368}{2020}

\bibitem{Rezai:2020}
\reference{Rezai Z}{\it The Astrophysical Journal}{\bf 902}{102}{2020}

\bibitem{Riess:2019}
\reference{Riess A. G., Casertano S, Yuan W, Macri L. M. and Scolnic D}{\it Astrophys. J.}{\bf 876}{85}{2019}

\bibitem{Ross:2015}
\reference{Ross A. J., Samushia L, Howlett C, Percival W. J., Burden  A and Manera M}{\it Mon. Not. Roy. Astron. Soc.}{\bf 449}{835}{2015}

\bibitem{Roy:2019}
\reference{Roy N and Bamba K}{\it Phys. Rev. D}{\bf 99}{123520}{2019}

\bibitem{Roy:2023}
\reference{Roy N}{\it General Relativity and Gravitation}{\bf 55}{115}{2023}

\bibitem{Ruiz:2015}
\reference{Ruiz E. J., Huterer D}{\it  Physical Review D}{\bf 91}{063009}{2015}

\bibitem{Sa:2021}
\reference{S\'a P M}{\it Physical Review D}{\bf 103}{123517}{2021}

\bibitem{Sadri:2019a}
\reference{Sadri E}{\it The European Physical Journal C}{\bf 79}{ 762}{2019}

\bibitem{Sadri:2019b}
\reference{Sadri E and Khurshudyan M}{\it International Journal of Modern Physics D}{\bf 28}{1950152}{2019}

\bibitem{Sadri:2020}
\reference{Sadri E, Khurshudyan Mi and Zeng D-f}{\it The European Physical Journal C}{\bf 80}{393}{2020}

\bibitem{Salzano:2021}
\reference{Salzano V, Pigozzo C, Benetti M et al.}{\it Journal of Cosmology and Astroparticle Physics}{\bf 09}{033}{2021}

\bibitem{Santos:2017}
\reference{Santos L, Zhao W, Ferreira E. G. M. \& Quintin J}{\it  Physical Review D}{\bf 96}{103529}{2017}

\bibitem{Schoneberg:2022}
\reference{Sch\"oneberg N, Franco Abell\'an G, P\'erez S\'anchez A, Witte S. J.,Poulin  V and Lesgourgues J}{\it Phys. Rept.}{\bf 984}{1}{2022}

\bibitem{Schutz}
\reference{Schutz B. F.}{Nature}{323}{310}{1986}

\bibitem{Schwarz:1978}
\reference{Schwarz G. E.}{\it Ann. Stat.}{\bf 6}{461}{1978}

\bibitem{Scoccimarro1998}
\reference{Scoccimarro R}{Mon. Not. Roy. Astron. Soc.}{299}{1097}{1998}

\bibitem{Scolnic:2022}
\reference{Scolnic D, Brout D, Carr A et al}{\it Astrophys J.}{\bf 938}{113}{2022}

\bibitem{Secco:2022}
\reference{Secco L. F. et al}{\it Phys. Rev. D}{\bf 105}{023515}{2022}

\bibitem{Shafieloo:2018}
\reference{Shafieloo A, Hazra D. K., Sahni V and Starobinsky A. A.}{\it Monthly Notices of the Royal Astronomical Society}{\bf 473}{2760}{2018}

\bibitem{Sharma:2020}
\reference{Sharma U. K., Varshney G and Dubey V. C.}{\it International Journal of Modern Physics D}{\bf 30}{2150021}{2020}

\bibitem{Sharov:2017}
\reference{Sharov G. S., Bhattacharya S, Pan S, Nunes R. C. and Chakraborty S}{\it Monthly Notices Royal Astronomical Society}{\bf 466}{3497}{2017}

\bibitem{Simons:2023}
\referencelink{https://simonsobservatory.org/}

\bibitem{Simpson:2010}
\reference{Simpson F}{\it Phys. Rev. D}{\it 82}{083505}{2010}

\bibitem{Sinha:2020}
\reference{Sinha S and Banerjee N}{\it The European Physical Journal Plus}{\bf 135}{779}{2020}

\bibitem{Sinha:2021}
\reference{Sinha S}{\it Physical Review D}{\bf 103}{123547}{2021}

\bibitem{Skara:2020}
\reference{Skara F and Perivolaropoulos L}{\it Phys. Rev.}{\bf D6}{101}{2020}

\bibitem{1312}
\reference{Sosa Almazan Maria Luisa, Izquierdo German}{Gen. Rel. Grav.}{\textbf{46}}{1759}{2014}

\bibitem{Spiegelhalter:2002}
\reference{Spiegelhalter D. J., Best N. G., Carlin B. P. \& Van Der Linde A}{\it Journal of the Royal Statistical Society: Series B (Statistical Methodology)}{\bf 64}{583}{2002}

\bibitem{gadget2}
\reference{Springel V}{Mon. Not. Roy. Astron. Soc.}{\textbf{364}}{1105-1134}{2005}

\bibitem{StageIV:2023}
\referencelink{https://cmb-s4.org/}

\bibitem{Starobinsky1985}
\reference{Starobinsky A. A.}{JETP Lett.}{42}{152-155}{1985} 

\bibitem{Tao:2020}
\reference{Tao Y}{\it Phys. Rev. D }{\bf 102}{083511}{2020}

\bibitem{Thipaksorn:2022}
\reference{Thipaksorn W, Sapa S and Karwan K}{\it Phys. Rev. D }{\bf 105}{063527}{2022}

\bibitem{1903}
\reference{Tsujikawa Shinji}{Phys. Rev. D}{100}{043510}{2019}

\bibitem{Yang69}
\reference{Vagnozzi S, Giusarma E, Mena O, Freese K, Gerbino M, Ho S and Lattanzi M}{Phys. Rev. D}{96}{123503}{2017}

\bibitem{Yang71}
\reference{Vagnozzi S, Dhawan S, Gerbino M, Freese K, Goo-bar A and Mena O}{Phys. Rev. D}{98}{083501}{2018}

\bibitem{Yang74}
\reference{Vagnozzi S, Brinckmann T, Archidiacono M, Freese K, Gerbino M, Lesgourgues J and Sprenger T}{JCAP}{1809}{001}{2018} 

\bibitem{Yang75}
\referenceA{Vagnozzi S}{arXiv:1907.08010}{2019}

\bibitem{Vagnozzi:2020}
\reference{Vagnozzi S, Visinelli L, Mena O and Mota D. F.}{\it Monthly Notices of the Royal Astronomical Society}{\bf 493}{1139}{2020}

\bibitem{vonMarttens:2019}
\reference{von Marttens R, Casarini L, Mota D. F. and Zimdahl W 2019}{\it Physics of the Dark Universe}{\bf 23}{100248}{2019}

\bibitem{Walter2018}
\reference{Walters A, Weltman A, Gaensler B. M., Ma Y. Z. and Witzemann A}{Astrophys. J.}{\textbf{856}}{65}{2018}

%\bibitem{wang1}
%\reference{B.~Wang, Y.~G.~Gong, E.~Abdalla}{Phys.Lett. B}{624}{141}{2005}

\bibitem{Wang:2016}
\reference{Wang B, Abdalla E, Atrio-Barandela F and Pav\'{o}n D}{\it Rept. Prog. Phys.}{\bf 79}{096901}{2016}

\bibitem{Wang:2017}
\reference{Wang S, Wang Y \& Li M }{\it Physics Reports}{\bf 696}{1}{2017}

\bibitem{Wang:2022}
\reference{Wang L-F, Zhang J-H, He D-Z, Zhang J-F and Zhang X}{\it Monthly Notices of the Royal Astronomical Society}{\bf 514}{1433}{2022}

%\bibitem{wang2}
%\reference{B.~Wang, C.-Y.~Lin, E.~Abdalla}{Phys.Lett. B}{637}{357}{2006}

%\bibitem{wang3}
%\reference{B.~Wang, Y.~G.~Gong, E.~Abdalla}{Phys.Rev. D}{74}{083520}{2006}

%\bibitem{wang4}
%\reference{B.~Wang, J.~D.~Zang, C.-Y.~Lin, E.~Abdalla, S.~Micheletti}{ Nucl.Phys.B}{778}{69}{2007}

%\bibitem{wang5}
%\reference{B.~Wang, C.-Y.~Lin, D.~Pavon, E.~Abdalla}{Phys.Lett. B}{662}{1}{2008}

\bibitem{Dai252}
\reference{Wei J. J., Wu X. F., and Gao H}{Astrophys. J.}{860}{L7}{018}

\bibitem{Weinberg}
\reference{Steven Weinberg}{Rev. Mod. Phys. }{61}{ 1 }{1989}

\bibitem{White1996}
\referenceB{White S. D. M.}{Cosmology and Large Scale Structure}{p349}{1996}

\bibitem{Wuensche2021}
\reference{Wuensche C. A., et al.}{Astron. Astrophys.}{664}{A15}{2022}

\bibitem{Dai2021}
\reference{Xiao D, Wang F and Dai Z}{Sci. China Phys. Mech. Astron.}{\textbf{64}}{249501}{2021}

\bibitem{Xiao2019}
\reference{Xiao L, An R, Zhang L, Yue B, Xu Y, Wang B}{Phys. Rev. D}{99}{023528}{2019}

\bibitem{Xiao:2019}
\reference{Xiao L, An R, Zhang L, Yue B, Xu Y and Wang B}{\it Physical Review D}{\bf 99}{023528}{2019}

\bibitem{Xiao:2020}
\reference{Xiao L, Zhang L, An R, Feng C and Wang B}{\it JACP}{\bf 01}{045}{2020}

\bibitem{Xiao:2021}
\reference{Xiao L, Costa A. A. and Wang B}{\it Monthly Notices of the Royal Astronomical Society}{\bf 510}{1495}{2021}

%\bibitem{xu1}
%\reference{X.~D.~Xu, J.~H.~He, B.~Wang}{Phys.Lett. B}{701}{513}{2011}

\bibitem{Xu:2018}
\reference{Xu X, Ma Y-Z and Weltman A}{\it Physical Review D}{\bf 97}{083504}{2018}

%\bibitem{xu2}
%\reference{X.~D.~Xu, B.~Wang, E.~Abdalla}{Phys.Rev. D}{85}{083513}{2012}

\bibitem{YangT:2020}
\reference{Yang T}{\it Physical Review D}{\bf 102}{083511}{2020}

\bibitem{Yang:2016}
\reference{Yang W, Li H, Wu Y \& Lu J}{\it  Journal of Cosmology and Astroparticle Physics}{\bf 10}{007}{2016}

\bibitem{Yang70}
\reference{Yang W, Nunes R. C., Pan S and Mota D. F.}{Phys. Rev. D}{95}{103522}{2017}

\bibitem{Yang:2017}
\reference{Yang W, Banerjee N \& Pan S}{\it  Physical Review D}{\bf 95}{123527}{2017}

\bibitem{Yang:2018a}
\reference{Yang W, Pan S \& Barrow J. D.}{\it Physical Review D}{\bf 97}{043529}{2018}

\bibitem{Yang:2018b}
\reference{Yang W, Pan S, Di Valentino E, Nunes R. C., Vagnozzi S and Mota D. F.}{\it Journal of Cosmology and Astroparticle Physics}{\bf 09}{019}{2018}

\bibitem{Yang:2018c}
\reference{Yang W, Pan S, Herrera R and Chakraborty S}{\it Physical Review D}{\bf 98}{043517}{2018}

\bibitem{Yang:2019a}
\reference{Yang W, Pan S and Paliathanasis A}{\it Monthly Notices of the Royal Astronomical Society}{\bf 482}{1007}{2019}

\bibitem{Yang:2019b}
\reference{Yang W, Vagnozzi S, Di Valentino E, Nunes R. C., Pan S and Mota D. F.}{\it Journal of Cosmology and Astroparticle Physics}{\bf 07}{037}{2019}

\bibitem{Yang:2019c}
\reference{Yang W,  Banerjee N, Paliathanasis A and Pan S}{\it Physics of the Dark Universe}{\bf 26}{100383}{2019}

\bibitem{Yang:2020a}
\reference{Yang W, Pan S, Nunes R. C. and Mota D. F.}{\it Journal of Cosmology and Astroparticle Physics}{\bf 04}{008}{2020}

\bibitem{Yang:2020b}
\reference{Yang W, Pan S, Di Valentino E, Wang B and Wang A}{\it Journal of Cosmology and Astroparticle Physics}{\bf 05}{050}{2020}

\bibitem{Yang:2021a}
\reference{Yang W, Pan S, Di Valentino E, Mena O and Melchiorri A}{\it Journal of Cosmology and Astroparticle Physics}{\bf 10}{008}{2021}

\bibitem{Yang:2022}
\reference{Yang W, Pan S, Mena O and Di Valentino E}{\it Journal of High Energy Astrophysics}{\bf 40}{19}{2023}

\bibitem{Zarandi:2021}
\reference{Zarandi H. R. M. and Ebrahimi E}{\it Monthly Notices of the Royal Astronomical Society}{\bf 511}{42}{2021}

\bibitem{Zhai:2023}
\reference{Zhai Y, Giar\'e W, van de Bruck C, Di Valentino E, Mena O and Nunes R C}{\it JCAP}{\bf 07}{032}{2023}

\bibitem{Zhang:2018}
\reference{Zhang J, An R, Liao S, Luo W, Li Z and Wang B}{\it Physical Review D}{\bf 98}{103530}{2018}

\bibitem{Zhang:2019}
\reference{Zhang J, An R, Liao S, Luo W, Li Z, Liao S and Wang B}{\it Astrophysics Journal Letters}{\bf 875}{L11}{2019}

\bibitem{Zhang2021}
\reference{Zhang J, et al.}{\it Astron. Astrophys.}{\bf 664}{A19}{2022}

\bibitem{Zhang:2021}
\reference{Zhang M, Wang B, Wu P-J, Qi J-Z, Xu Y, Zhang J-F and Zhang X}{\it Astrophysics Journal}{\bf 918}{56}{2021}

\bibitem{Zhang2022}
\reference{Zhang B}{\it Reviews of Modern Physics}{\bf 95}{035005}{2023}

\bibitem{Zhao:2020}
\reference{Zhao M. M., Guo R. Y., He D. Z., Zhang J. F. and Zhang X}{\it Science China Physics, Mechanics \& Astronomy}{\bf 63}{230412}{2020}

\bibitem{Zhao:2022}
\reference{Zhao Y, Liu Y, Liao S, Zhang J, Liu X and Du W}{\it Month. Not. Roy. Astron. Soc.}{\bf 523}{5962}{2023}

\bibitem{Dai253}
\reference{Zhao Z. W., Li Z. X., Qi J. Z., Gao H, Zhang J. F., and Zhang X}{Astrophys. J.}{903}{83}{2020}

\bibitem{Zhao2022}
\reference{Zhao Z W, Wang L F, Zhang J. G., Zhang J. F. and Zhang X}{JCAP}{\bf 04}{022}{2023}

\bibitem{Zheng:2017}
\reference{Zheng X, Biesiada M, Cao S, Qi J \&  Zhu Z-H}{\it Journal of Cosmology and Astroparticle Physics}{\bf 10}{030}{2017}

\bibitem{Zhou2014}
\reference{Zhou B, Li X, Wang T, Fan Y. Z. and Wei D. M.}{Phys. Rev. D}{\textbf{89}}{107303}{2014}

%\bibitem{zhou}
%\reference{J.~Zhou, B.~Wang, D.~Pavon, E.~Abdalla}{Mod.Phys.Lett. A}{24}{1689}{2009}

\bibitem{Zhu2022}
\reference{Zhu Liang-Gui, Hu Yi-Ming, Wang Hai-Tian, Zhang Jian-dong, Li Xiao-Dong, Hendry Martin, Mei Jianwei}{Phys. Rev. Res.}{\textbf{4}}{013247}{2022}

\bibitem{Zumalacarregui:2013pma}
\reference{Zumalacarregui, Miguel and Garcia-Bellido, Juan}{Phys. Rev. D}{89}{064046}{2014}. 

\end{thebibliography}

\end{document}

